VURF: A General-purpose Reasoning and Self-refinement Framework for Video Understanding

Recent studies have demonstrated the effectiveness of Large Language Models (LLMs) as reasoning modules that can deconstruct complex tasks into more manageable sub-tasks, particularly when applied to visual reasoning tasks for images. In contrast, this paper introduces a Video Understanding and Reasoning Framework (VURF) based on the reasoning power of LLMs. Ours is a novel approach to extend the utility of LLMs in the context of video tasks, leveraging their capacity to generalize from minimal input and output demonstrations within a contextual framework. We harness their contextual learning capabilities by presenting LLMs with pairs of instructions and their corresponding high-level programs to generate executable visual programs for video understanding. To enhance the program's accuracy and robustness, we implement two important strategies. \emph{Firstly,} we employ a feedback-generation approach, powered by GPT-3.5, to rectify errors in programs utilizing unsupported functions. \emph{Secondly}, taking motivation from recent works on self-refinement of LLM outputs, we introduce an iterative procedure for improving the quality of the in-context examples by aligning the initial outputs to the outputs that would have been generated had the LLM not been bound by the structure of the in-context examples. Our results on several video-specific tasks, including visual QA, video anticipation, pose estimation, and multi-video QA, illustrate these enhancements' efficacy in improving the performance of visual programming approaches for video tasks.

==> tables/ground_trans.tex <==
\begin{table}[!t]
    \centering
    \begin{minipage}[t]{0.48\textwidth} % Adjust width as needed
        \centering
        \caption{\emph{\textbf{Demostration of VURF without the influence of an imperfect module.}} We evaluated our Video Question Answering task first using an imperfect temporal localization module (GROUND) and then the actual ground truths.}
        \vspace{1em}
        \label{tab: ground}
        \setlength{\tabcolsep}{6pt} % Default value: 6pt
        \renewcommand{\arraystretch}{1} % Default value: 1
        \scalebox{0.85}[0.85]{
        \begin{tabular}{ccc}
            \toprule
            Dataset & No Ground Truth & Ground Truth \\
            \toprule 
            NextQA \cite{xiao2021next} & 61.4\% & 65.2\% \\
            \bottomrule
        \end{tabular}}
    \end{minipage}%
    \hfill % To insert a horizontal space between the tables
    \begin{minipage}[t]{0.48\textwidth} % Adjust width as needed
        \centering
        \caption{\emph{\textbf{Effect of using transcripts from the Social-IQ QA dataset}.}}
        \label{tab: social}
        \setlength{\tabcolsep}{6pt} % Default value: 6pt
        \renewcommand{\arraystretch}{1} % Default value: 1
        \scalebox{0.85}[0.85]{
        \begin{tabular}{ccc}
            \toprule
            Dataset & Baseline & With transcripts \\
            \toprule
            Social-IQ-2.0 \cite{zadeh2019social} & 48.1\% & 51.6\% \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
\end{table}


==> tables/llm.tex <==
\begin{table}[!t]
        \caption{\emph{\textbf{Comparison with multiple LLMs}}, both open source models and other GPT model versions.}
         % \vspace{-1em}
        \label{tab: llm}
	\centering\small
		% \setlength{\tabcolsep}{7.5pt}
            \setlength{\tabcolsep}{9.3pt} % Default value: 6pt
            \renewcommand{\arraystretch}{1} % Default value: 1
        \scalebox{0.85}[0.85]{
        \begin{tabular}{ccc}
            \toprule
            \textbf{LLM} & STAR & Social-IQ-2.0\\
            \toprule
            \textbf{GPT-3.5-turbo-instruct (original)} & $47.2\%$ & $51.6\%$ \\
            \textbf{GPT-4}  & $43.5\%$ & $49.1\%$ \\
            \midrule
            \textbf{CodeLlama-7b} & $10.0\%$ & $5.0\%$ \\
            \textbf{CodeLlama-7b-Instruct} & $42.3\%$ & $48.4\%$ \\
            \textbf{Code-T5} & $0\%$ & $0\%$ \\
            \bottomrule
        \end{tabular}}
        % \vspace{0.7em}
\end{table}

==> tables/nextqa_ground.tex <==
\begin{table}[!t]
    \caption{\emph{\textbf{Demostration of VURF without the influence of an imperfect module.}} We evaluated our Video Question Answering task first using an imperfect temporal localization module (GROUND) and then the actual ground truths.}
        \vspace{1em}
        \label{tab: ground}
	\centering\small
		% \setlength{\tabcolsep}{7.5pt}
            \setlength{\tabcolsep}{9.3pt} % Default value: 6pt
            \renewcommand{\arraystretch}{1} % Default value: 1
		\scalebox{0.85}[0.85]{
		\begin{tabular}{ccc}
                    \toprule
				Dataset & No Ground Truth & Ground Truth \\
                    \toprule 
                    NextQA \cite{xiao2021next} & 61.4\% & 65.2\% \\

		      % \toprule
	   \bottomrule
	\end{tabular}}
	% \vspace{0.7em}
\end{table}


==> tables/social_transcript.tex <==
\begin{table}[!t]
    \caption{\emph{\textbf{Effect of using transcripts from the Social-IQ QA dataset}.}}
    % \vspace{-1em}
    \label{tab: social}
    \centering\small
    \setlength{\tabcolsep}{9.3pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1} % Default value: 1
    \scalebox{0.85}[0.85]{
    \begin{tabular}{ccc}
        \toprule
	Dataset & Baseline & With transcripts \\
        \toprule
        Social-IQ-2.0 & 48.1\% & 51.6\% \\
        % \toprule
	\bottomrule
    \end{tabular}}
    % \vspace{0.7em}
\end{table}
